Rigorous body-order approximations of an electronic structure potential energy landscape

We show that the local density of states (LDOS) of a wide class of tight-binding models has a weak body-order expansion. Specifically, we prove that the resulting body-order expansion for analytic observables such as the electron density or the energy has an exponential rate of convergence both at finite Fermi-temperature as well as for insulators at zero Fermi-temperature. We discuss potential consequences of this observation for modelling the potential energy landscape, as well as for solving the electronic structure problem.

==> diagrams/finiteTempContour.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.8,xscale=.8]
%uncomment if require: \path (0,388); %set diagram left start at 0, and has height of 388

%Shape: Rectangle [id:dp16117257917452332] 
\draw  [draw opacity=0][fill={rgb, 255:red, 231; green, 231; blue, 231 }  ,fill opacity=1 ] (22.8,46.2) -- (631.8,46.2) -- (631.8,337.2) -- (22.8,337.2) -- cycle ;
%Rounded Rect [id:dp46905161902154524] 
\draw  [color={rgb, 255:red, 34; green, 4; blue, 230 }  ,draw opacity=1 ][line width=1.5]  (150.45,168.3) .. controls (150.45,126.49) and (184.34,92.6) .. (226.15,92.6) -- (432.1,92.6) .. controls (473.91,92.6) and (507.8,126.49) .. (507.8,168.3) -- (507.8,215.5) .. controls (507.8,257.31) and (473.91,291.2) .. (432.1,291.2) -- (226.15,291.2) .. controls (184.34,291.2) and (150.45,257.31) .. (150.45,215.5) -- cycle ;
%Shape: Rectangle [id:dp7971907261280502] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (251.8,189.2) -- (402.3,189.2) -- (402.3,202.2) -- (251.8,202.2) -- cycle ;
%Straight Lines [id:da6643812855646833] 
\draw [line width=2.25]    (29.3,186.16) -- (49,208.96) ;
%Straight Lines [id:da22265806345974726] 
\draw [line width=2.25]    (28.3,207.16) -- (50.65,189.06) ;
%Straight Lines [id:da10564706341160068] 
\draw [line width=2.25]    (608.3,186.16) -- (628,208.96) ;
%Straight Lines [id:da5148925700334295] 
\draw [line width=2.25]    (607.3,207.16) -- (629.65,189.06) ;
%Straight Lines [id:da48627196611769796] 
\draw    (53.8,197.2) -- (143.8,197.2) ;
\draw [shift={(146.8,197.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(50.8,197.2)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3449812267999517] 
\draw    (188.78,273.94) -- (247.82,206.46) ;
\draw [shift={(249.8,204.2)}, rotate = 491.19] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(186.8,276.2)}, rotate = 311.19] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da269042026868894] 
\draw    (517.8,198.2) -- (607.8,198.2) ;
\draw [shift={(610.8,198.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(514.8,198.2)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da190230122751067] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (22.8,46.2) -- (631.8,46.2) ;
%Straight Lines [id:da6675421576866121] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (22.8,337.2) -- (631.8,337.2) ;
%Straight Lines [id:da48944498415079263] 
\draw [line width=2.25]    (316.3,9.16) -- (336,31.96) ;
%Straight Lines [id:da7322281043225736] 
\draw [line width=2.25]    (315.3,30.16) -- (337.65,12.06) ;
%Straight Lines [id:da3851306171981952] 
\draw [line width=2.25]    (316.3,348.16) -- (336,370.96) ;
%Straight Lines [id:da46349345794556185] 
\draw [line width=2.25]    (315.3,369.16) -- (337.65,351.06) ;

% Text Node
\draw (495,290) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$\mathscr{C}$};
% Text Node
\draw (29,166.4) node [anchor=north west][inner sep=0.75pt]    {$-1$};
% Text Node
\draw (606,167.4) node [anchor=north west][inner sep=0.75pt]    {$+1$};
% Text Node
\draw (92,176.4) node [anchor=north west][inner sep=0.75pt]    {$\mathsf{d}$};
% Text Node
\draw (208,220.4) node [anchor=north west][inner sep=0.75pt]    {$\mathfrak{d}$};
% Text Node
\draw (558,177.4) node [anchor=north west][inner sep=0.75pt]    {$\mathsf{d}$};
% Text Node
\draw (30,50.4) node [anchor=north west][inner sep=0.75pt]    {$|\mathrm{Im} \ z|< \sqrt{\mathsf{d}}\log\left( 1+\frac{\pi }{2\tilde{\beta }}\right)$};
% Text Node
\draw (342,5.4) node [anchor=north west][inner sep=0.75pt]    {$\tilde{\mu } +\frac{\pi i}{2\tilde{\beta }}$};
% Text Node
\draw (342,344.4) node [anchor=north west][inner sep=0.75pt]    {$\tilde{\mu } -\frac{\pi i}{2\tilde{\beta }}$};


\end{tikzpicture}


==> other/articles.tex <==

\section{Introduction}
\begin{itemize}

\item Drawbacks of using a locality ansatz for the physical properties of the system: long range electrostatic interactions play a key role in .... The slow decay of the Coulomb interaction hampers convergence of a local machine learning scheme  

\item LODE \cite{Grisafi2019}:
\begin{itemize}
    \item non-self-consistent, 
    
    \item ``introducing nonlocal representations of the system, which are remapped as feature vectors'', 
    
    \item ``By combining a representation of the system that is sensitive to long-range correlations with the transferability of an atom-centered additive model, this method outperforms current state-of-the-art machine-learning schemes''. 

    \item gas of point charges:
    \begin{itemize}
        \item  random configurations of point charges such that system is overall neutral, \item use Ewald summation to get electrostatic energy of the configuration
        \item simple Gaussian process regression to learn the mapping from features to energy for SOAP and LODE features with different parameters 
    \end{itemize}
   
   \item binding curves for charged dimers:
    \begin{itemize}
        \item at least one of the two monomers in each dimer configuration has a net charge (focuses on a problem for which electrostatics plays a key role)
        
        \item for each dimer, the dataset has multiple configurations with different distances between the monomers
        
        \item DFT calculations $\rightarrow$ binding curves for each configuration
        
        \item isolated monomers also contained in the dataset (has knowledge of the dissociation limit)
    \end{itemize}
\end{itemize}

\item BpopNN (Becke population Neural Network) \cite{Xie2020}: 
\begin{itemize}
    \item self-consistent but not long-range (atom centred Gaussian proxy densities approximate the electrostatic potential),
    
    \item learn population $\mapsto$ DFT energy (using constrained DFT \& neural network). Here, the loss function involves the energy, forces and derivatives of the energy with respect to the populations.
    
    \item then minimise with respect to these populations (using CG method) $\rightarrow$ results in a SCF 

    \item Lithium hydride clusters
    \begin{itemize}
        \item data: clusters of varying sizes, relatively widely separated molecules (``sparse'') and denser roughly cubic structures (``non-sparse''). DFT geometry optimisation of samples gives more data. For ``non-sparse'' structures, \textit{ab initio} MD simulations are also used to generate more data,
        
        \item training/validation split 95/5 + tuned hyperparameters,
        
        \item then considered larger clusters to test transferability
    \end{itemize}
    
\end{itemize}

    \iffalse\item ``Interatomic potentials for ionic systems with density functional accuracy based on charge densities obtained by a neural network''
    \begin{itemize}
        \item consider a site energy description
        \[
            E = \sum_i \left( E_i + \chi_i q_i + \frac{1}{2} J_{ii} q_i^2 \right) + \frac{1}{2}\in\int \frac{\rho(r)\rho(r^\prime)}{|r - r^\prime|}
        \] 
        
        \item learn the mapping from features (based on atom centred symmetry functions) $\mapsto \{\chi_i\}$ (the electronegativity of the atom)
        
        \item minimise energy w.r.t.~charges $\{q_i\}$ gives the ground state charges
        
        \item calculate total energy and forces 
        
        \item application: Sodium chloride clusters
    \end{itemize}
     \fi

\end{itemize}


==> other/extra_comments.tex <==
\newpage

\section*{\jtedit{(extra comments)}}

\jt{some references:}

\cite{Grisafi2019} Grisafi, Ceriotti. Incorporating long-range physics in atomic-scale machine learning. 2019: (LODE)
%
\begin{itemize}
    \item introduces nonlocal representations of the system (SOAP + extra features)
    
    \item Gaussian process regression to learn mapping from features to energy
\end{itemize}

\cite{GrisafiEtAl2019} Transferable Machine-Learning Model of the Electron Density, 2019:
%
\begin{itemize}
    \item decompose electron density into atom centred contributions
    \[
        \rho(\bm r) = \sum_i \rho_i(\bm r) = \sum_{ik} c_{nlm}^i \phi_{nlm}(\bm r - \bm r_i).
    \]
    \item Gaussian process regression for the coefficients using only nuclei positions and targetting only the electron density 
\end{itemize}

\cite{Xie2020} Incorporating Electronic Information into Machine Learning Potential Energy Surfaces via Approaching the Ground-State Electronic Energy as a Function of Atom-Based Electronic Populations. 2020: (BpopNN Becke population NN)
%
\begin{itemize}
    \item use constrained DFT calculations together with NN to learn the mapping: ``electron populations'' to DFT energy
    
    \item loss function includes energy, forces and derivatives of energy wrt populations
    
    \item Then, minimise energy wrt populations (SCF iteration)
\end{itemize}


(other notes)
%
\begin{enumerate}
    \item $\bm r_\ell - \bm r_\ell^\prime = \ep_\ell$ with $|\ep|$ sufficiently small
    %
    \[
        |h_{\ell k}(\bm r_{\ell k}) - h_{\ell k}( \bm r_{\ell k}^\prime )| 
        %
        = |\nabla h_{\ell k}( \xi ) \cdot (\ep_\ell - \ep_k)|
        %
        \lesssim |\ep| e^{-\gamma_0 r_{\ell k}}
    \]
    %
    similarly, $|\sum_m t(\bm r_{\ell m}, \bm{r}_{km}) - t(\bm r^\prime_{\ell m}, \bm{r}^\prime_{km})| \lesssim |\ep| e^{-\gamma r_{\ell k}}$,
    
    Therefore, 
    \[
        \mathrm{dist}(\sigma(\Ham(\bm r)),\sigma(\Ham(\bm r^\prime)) ) 
        %
        \leq \|\Ham(\bm r) - \Ham(\bm r^\prime)\|_{\ell^2 \to \ell^2}
        %
        \lesssim |\ep|
    \]
    (Hausdorff distance, Kato Thm~4.10, pg.~291)
     
    \item Point defect - finite rank update result
    
    \item More generally, if $P \coloneqq \Ham(\bm r) - \Ham(\bm r^\prime)$ is compact, then there exists $P_n$ finite rank, s.t.~$\lim_{n\to\infty}\|P - P_n\|_{\ell^2\to\ell^2} \to 0$ and so can combine the above two cases to get the same result...
\end{enumerate}


\jt{This is unnecessary now}




\begin{proof}[Proof of Theorem~\ref{thm:bodyOrder_interpolation_discrete}]
    We consider 
    %
    $\widetilde{E} = E \cup \{\lambda_j\}$ 
    %
    where $E$ is the set introduced in Theorem~\ref{thm:bodyOrder_interpolation} and $\{\lambda_j\}$ is a set of isolated eigenvalues.
    
    We first observe that, since $\mathrm{cap}(E)$ is non-zero,
    %
    $V_E = V_{\widetilde{E}}$, $\mu_{\widetilde{E}} = \mu_E$
    %
    and thus $g_{\widetilde{E}} = g_E$. Therefore, uniformly on compact subsets of
    %
    $\mathbb C \setminus \widetilde{E}$,
    %
    we have \cref{eq:lim_ell}.
    
    We conclude by applying \cref{eq:Hermite} with 
    %
    $X_N \supset \{\lambda_j\}$ 
    %
    and contours
    %
    $\mathscr C_j \coloneqq \{z\in\mathbb C\colon g_E(z) = \log r_j\}$ 
    %
    with $r_2 > r_1 > 1$. Since $\{\lambda_j\}$ are interpolation points, contributions to the integral \cref{eq:Hermite} from discrete eigenvalues $\lambda_j$ are zero (that is,
    %
    \[
        \big( O^\beta(\lambda_j) - I_NO^\beta(\lambda_j) \big) |[\psi_j]_\ell|^2 = 0
    \]
    %
    for each $\lambda_j$, where $\psi_j$ are corresponding normalised eigenvectors). This means that the integration contour $\mathscr C_1$ does not need to encircle all (or any) of the discrete eigenvalues $\{\lambda_j\}$.
    
    Adding finitely many discrete points to the interpolation set does not affect the limiting measure and so if Theorem~\ref{thm:bodyOrder_interpolation} holds for some sequence of interpolation points $X_N$, then Theorem~\ref{thm:bodyOrder_interpolation_discrete} holds for 
    %
    $\widetilde{X}_N \coloneqq X_N \cup \{\lambda_j\}$.
\end{proof}


\jt{classical body order expansion}

However, the convergence of the classical body-order expansion is not immediate:
\begin{align}\label{othernotes}
    O_\ell(\bm r) - 
    %
    \sum_{n=0}^N 
    \sum_{\above
        {k_1,\dots,k_n \not= \ell}
        {k_1 < \dots < k_n}
    }
    V^{(n)}( \bm{r}_{\ell k_1}, \dots, \bm{r}_{\ell k_n} )
    %
    =  
    \sum_{n=0}^N 
    \sum_{\above
        {k_1,\dots,k_n \not= \ell}
        {k_1 < \dots < k_n}
    }
    (V_{nN} - V^{(n)})( \bm{r}_{\ell k_1}, \dots, \bm{r}_{\ell k_n} )
    %
    + O(e^{-\gamma_N N})
\end{align}
The convergence of the classical body-order expansion follows if 
\[
    \bigg( 
        \sum_{n=0}^N 
        \sum_{\above
            {k_1,\dots,k_n \not= \ell}
            {k_1 < \dots < k_n}
        } 
        c_n(k_1,\dots,k_n)
    \bigg) e^{-\gamma_N N} \to 0
\]

Probably the best we can hope for is
\[
    c_n(k_1,\dots,k_n) \lesssim e^{-\gamma d(\ell ; k_1,\dots,k_n )}
\]
where $d(\ell ; k_1,\dots,k_n )$ is the length of the shortest path $\ell \to \ell$ of length $n+1$ visiting $k_1,\dots,k_n$. 

Simplify: $c_n(k_1,\dots,k_n)$ bounded for $k_1,\dots,k_n \in K$ where $|K| = N_\mathrm{at}$ and $c_n$ zero otherwise, then 
\[
   \sum\sum c_n \lesssim \sum_{n=0}^N \frac{N_{\mathrm{at}}^n}{n!} \approx e^{N_\mathrm{at}}
\]
for large body-order.




\section*{Adding $[-\ep,\ep]$ to the interpolation set}

Take $\mu = 0$ and suppose that $E = [-1,a]\cup[b,1]$ and the interpolation set is given by the union of Fekete points on $E$ with density $\alpha$ and Chebyshev points on $[-\ep,\ep]$ with density $1-\alpha$. Then, the corresponding node polynomial satisfies: for $\xi \in \mathscr C_\gamma \coloneqq \{ g_E = \gamma \}$ with $\gamma < g_E( i\pi \beta^{-1})$, we have
%
\[
    \lim_{N\to\infty} \left|
        \frac{\ell_N(z)}{\ell_N(\xi)}
    \right|^{\frac{1}{N}}
    %
    = e^{\alpha\big[ 
        g_E(z) - g_E(\xi)
    \big]} 
    e^{(1-\alpha) \big[ 
        g_{[-1,1]}(z/\ep) - g_{[-1,1]}(\xi/\ep)
    \big]}
\]
%

We wish to choose $\alpha > 0$ so that we preserve the asymptotic behaviour for $z \in E$: for example, choose $\alpha$ such that
%
\[
    -\alpha \gamma
    %
    + (1 -\alpha)\big[ 
        g_{[-\ep,\ep]}(z) - 
        g_{[-\ep,\ep]}(\xi)
    \big]
    %
    \leq - \frac{1}{2} \alpha \gamma
\]
%
for all $z \in E$ and $\xi \in \mathscr C_\gamma$. In particular, we have
%
\[
    \alpha \gamma
    %
    + (1 -\alpha)\big[ 
        g_{[-\ep,\ep]}(i\pi\beta^{-1}) - 
        g_{[-\ep,\ep]}(\pm1)
    \big]
    %
    \geq  \frac{1}{2} \alpha \gamma
\]
%
where $\pm1$ maximises $g_{[-\ep,\ep]}$ on $E$ and so it suffices to choose $\alpha$ such that
%
\[
    \frac{1}{2} \frac{\alpha}{1-\alpha} \gamma + g_{[-\ep,\ep]}(i\pi\beta^{-1}) = \frac{1}{\ep} 
    %
    \quad \bigg( \geq g_{[-\ep,\ep]}(\pm1) \bigg)
\]
%
(true for $\ep < \frac{1}{\sqrt{2}}$). 
%


But now, when $z\in [-\ep,\ep]$, we obtain the asymptotic exponent
%
\begin{align}
    \alpha \bigg[ 
        g_E(z) - g_E(\xi) 
        - 
        \frac{1-\alpha}{\alpha}
        g_{[-1,1]}(\xi/\ep)
    \bigg]
    %
    &= \alpha \bigg[ 
        g_E(z) - g_E(\xi) 
        - 
        \frac
            {\ep g_{[-\ep,\ep]}(\xi)}
            {2 \big( 
                1 - \ep g_{[-\ep,\ep]}(i\pi\beta^{-1}) 
            \big)}
    %
    \bigg] \\
    %
    &\sim \alpha \bigg[ 
        g_E(z) - g_E(\xi) 
        - \frac
            {\beta^{-1}}
            {1 - \beta^{-1}}
    \bigg]
\end{align}
%
for $\xi = i \pi\beta^{-1}$.

That is, the choice of $\ep>0$ which would lead to improved convergence is negated by the fact that $\alpha = \alpha(\ep)$ must be chosen close to $1$.

\section*{``Potential Theory Interpolation'' with $E = [-1,a]\cup[-\ep,\ep]\cup[b,1]$}

The Green's function in this case is 
%
\begin{align}
    g_E(z) = \mathrm{Re} \int_1^z 
    \frac
        {(\zeta - z_3) (\zeta - z_6)}
        {\sqrt{\zeta + 1}\sqrt{\zeta -a}\sqrt{\zeta +\ep}
        \sqrt{\zeta - \ep}\sqrt{\zeta -b}\sqrt{\zeta - 1}} 
    \mathrm{d\zeta}
\end{align}
%
where $z_3 \in (a,-\ep)$ and $z_6 \in (\ep, b)$ with $z_{3,6}(\ep)\to z_{3,6}$ as $\ep \to 0$.

Simplify and set $a = -\mathsf{g}$, $b = \mathsf{g}$ and $\min\{-z_3,z_6\} = \tau \mathsf{g}$. The asymptotic convergence rate on $E$ is given by $g_E(i\pi\beta^{-1})$:
%
\begin{align}
    \frac
        {\beta^{-1}}
        {(\beta^{-2} + 1)(\beta^{-2} + \mathsf{g}^2)}
    \frac
        {\beta^{-2} + (\tau\mathsf{g})^2}
        {\beta^{-2} + (\ep\mathsf{g})^2}
    %
    \leq g_E(i\pi\beta^{-1}) 
    %
    \leq \frac{\beta^{-1}}{\ep \mathsf{g}^2} (\beta^{-2} + \mathsf{g}^2) 
    %\frac
    %    {\beta^{-1}}
    %    {\ep \mathsf{g}} 
    %
\end{align}
%
\jt{this isn't quite right}

\section*{Zero Fermi-Temperature}

Idea: compare zero temperature quantity with smooth smearing function and approximate the smooth function.

Instead: For zero temperature quantity $O_\ell(\bm r, v)$, take a smooth approximation $z \mapsto O^\beta(z)$ and get
\begin{align}
    \big|
        O_\ell(\bm r, v) - I_N O^\beta_\ell(\bm r, v) 
    \big|
    %
    &\leq \underbrace{\sup_{z\in\sigma(\Ham)} | O(z) - O^\beta(z) |}_{\eqqcolon s_\beta} 
    %
    + \underbrace{\sup_{z\in\sigma(\Ham)} | O^\beta(z) - I_N O^\beta(z) |}_{\eqqcolon\ep_{\beta,N}}.
\end{align}
%

\textit{(i)} Using interpolation with points from potential theory + Hermite integral formula, we have
%
\begin{align}
    \ep_{\beta,N} \lesssim 
    %
    \max_{\xi \in \mathscr C_\gamma} |O^\beta(\xi)| \, 
    %
    e^{-\gamma_N N} 
\end{align}
with $\gamma_N \to \gamma$ and $\mathscr C_\gamma \coloneqq \{ g_E = \gamma\}$.

\textit{(ii)} Using Chebyshev projection (or interpolation in Chebyshev points): $O^\beta(z) = \sum_{n=0}^\infty a_n T_n(z)$ with $|a_n| \leq 2 \sup_{z \in E_\rho} |O^\beta(z)| \, \rho^{-n}$ where $O^\beta$ is analytic on the $\rho-$Bernstein ellipse $E_\rho$ [ellipse with foci points $\pm1$ and semi-minor axis $\frac{1}{2}(\rho - \rho^{-1})$ and semi-major axis $\frac{1}{2}(\rho + \rho^{-1})$]. Therefore,
\[
    |O^\beta(z) - \Pi_N O^\beta(z) | \leq 2 \sup_{z \in B_\rho} |O^\beta(z)| \, \frac{\rho^{-N}}{1-\rho}
\]
(can replace the $2$ with $4$ for interpolation in Chebyshev points). This approach is probably better in this context because we get pre-asymptotic estimates

\subsection{Fermi-Dirac smearing} [see old manuscript for full results and proofs]
    
    Fermi-Dirac: the smearing function error is
    %
    $s_\beta \sim \beta^{-1} e^{-\mathsf{g}^\mathrm{def} \beta}$ \cite{OrtnerThomas2020:pointdefs}.
    %
    Shift and scale spectrum to $[-1,1]$ and let $\Pi_N$ be the degree $N$ Chebyshev projection on $[-1,1]$. Then, since the coefficients in the Chebyshev expansion decay exponentially as $\beta^{-1}$, we get 
    %
    $\ep_{\beta N} \sim e^{-\beta^{-1} N}$
    %
    and choosing 
    %
    $\mathsf{g}^\mathrm{def} \beta = \beta^{-1} N$,
    %
    we get
    %
    $\beta_N = \sqrt{\frac{N}{\mathsf{g}}}$
    %
    [or, slightly better: $\mathsf{g} \beta_N^2 + \beta_N \log \beta_N = N$] and   
    \[
        \big|
            O_\ell(\bm r, v) - \Pi_N O^\beta_\ell(\bm r, v) 
        \big|
        %
        \lesssim e^{- \sqrt{\mathsf{g}N}}
    \]

\subsection{Gauss error function}

Use the following entire function:
%
\begin{align}
    O^\beta(z) &\coloneqq \frac{1}{2}\big( 1 - \mathrm{erf}(\beta z) \big)
    %
    \quad \text{where} \quad
    %
    \mathrm{erf}(z) \coloneqq  \frac{2}{\sqrt{\pi}} \int_0^z e^{-t^2} \mathrm{d}t
\end{align}

A simple calculation reveals [$|O^\beta(ix)| \leq C e^{x^2}$] 
\[
    s_\beta \sim e^{-(\mathsf{g}\beta)^2}, 
    %
    \quad \textrm{and} \quad
    % 
    \ep_{\beta,N} \sim e^{(\rho\beta)^2} \rho^{-N}
\]
Therefore, balancing the error, leads to the requirement that
%
\begin{gather}
    \rho > 1, \quad \alpha \in (0,1), \quad \text{and} \quad 
    \frac{\alpha \rho^2}{1 -\alpha} \leq \frac{\alpha N \log \rho}{\beta^2} \leq \mathsf{g}^2
\end{gather}
%
and a rate $\sim \rho^{-\alpha N}$.

In particular, by choosing 
%
\begin{align}
    \alpha, \beta, \rho \colon \quad 
    %
    \beta^2 = \frac{N}{1 + \mathsf{g}^2} \beta_0, \quad
    %
    \alpha = \frac{\mathsf{g}^2}{1 + \mathsf{g}^2} \alpha_0, \quad 
    %
    \rho = e^{\frac{\beta_0}{\alpha_0}}, \quad
    %
    \alpha_0 \in (0,1), \quad
    %
    \beta_0 > 0,
\end{align}
%
we get
%
\[
    \mathrm{error} \sim e^{-\frac{\mathsf{g}^2}{1 + \mathsf{g}^2} \beta_0 N}, \quad 
    %
    \beta_0 \leq \frac{\alpha_0}{2} \log \left(
        \frac
            {1 + \mathsf{g}^2(1 - \alpha_0)}
            {\alpha_0}
    \right), \quad
    %
    \alpha_0 \in (0,1),
\]
%
with exponent $\sim \mathsf{g}^2$ as $\mathsf{g} \to 0$. (This is worse than our zero temperature interpolation results)

\subsection{Higher order Methfessel–Paxton methods}

If we use the order $p$ M-P method, we obtain
\[
    s_\beta + \ep_{\beta N} \sim \beta^{-2(p+1)} e^{-(\beta\mathsf{g})^2} + (\beta\rho)^{2p-1} e^{(\beta\rho)^2} \rho^{-N}
\]
[which looks very similar to previous section]

(extra convergence factor is negated since the approximations blow up quicker along $i\mathbb R$.

\section*{Small Perturbations}

Suppose the spectrum is contained in $[-1+\ep,a-\ep] \cup \{\lambda\} \cup [b+\ep,1-\ep]$ and consider small perturbation so that the spectrum is contained in $[-1, a] \cup (\lambda-\ep,\lambda+\ep)\cup [b,1]$ with $\mu \not\in (\lambda-\ep,\lambda+\ep)$.
%
Existing results (with interpolation points in $[-1,a]\cup[b,1]$) gives
\[
    |O_\ell(\bm r) - I_N O_\ell(\bm r)| \lesssim e^{-(\gamma_N - \eta_N) N}
\]
where $\gamma_N - \eta_N \to \gamma - \eta \sim \mathsf{g}^\mathrm{def} + \beta^{-1}$ as $\mathsf{g} + \beta^{-1} \to 0$ (where $\eta = \max\{g_E(\lambda-\ep), g_E(\lambda+\ep)\}$ and $\mathsf{g}^\mathrm{def} = \min\{ |\lambda + \ep - \mu|, |\lambda - \ep - \mu|\}$).

Putting interpolation points in $(\lambda-\ep,\lambda+\ep)$ gives:
\[
    |O_\ell(\bm r) - I_N O_\ell(\bm r)| \lesssim e^{-\widetilde{\gamma}_N N}
\]
with $\widetilde{\gamma}_N \to \widetilde{\gamma} \sim \sqrt{\mathsf{g}_-}\sqrt{\mathsf{g}_+} + \beta^{-1}$ as $\mathsf{g} + \beta^{-1} \to 0$ where $\mathsf{g}_- = \max_{z \in \sigma(H)\colon z< \mu} |z - \mu|$ and $\mathsf{g}_+ = \max_{z \in \sigma(H)\colon z> \mu} |z - \mu|$. (for a single isolated eigenvalue, this is $\sqrt{\mathsf{g}^\mathrm{def}} \sqrt{\mathsf{g}}$ instead of $\mathsf{g}^\mathrm{def}$)

\subsection{Consider $E = [-1,a]\cup[b,1]$ and $E^\prime = [\lambda-\ep,\lambda+\ep]$}

Put interpolation points in $E^\prime \coloneqq (\lambda-\ep,\lambda+\ep)$ with density $\alpha$ and $E \coloneqq [-1,a] \cup [b,1]$ with density $1-\alpha$. Then, for $z\in \mathbb R$ and $\xi \in \mathscr C$, we have
%
\begin{align}
    \lim_{N\to\infty} \left|
        \frac{\ell_N(z)}{\ell_N(\xi)}
    \right|^{\frac{1}{N}}
    %
    = e^{(1-\alpha)\big[ 
        g_E(z) - g_E(\xi)
    \big]} 
    e^{\alpha\big[ 
        g_{E^\prime}(z) - g_{E^\prime}(\xi)
    \big]}
\end{align}
%
Choose $\alpha > 0$ sufficiently small such that the error on $E$ is still given by the Green's function for $E$: For $z\in E$ and $g_E(\xi) = \gamma$, 
\[
    -(1 - \alpha) \gamma + \alpha( g_{E^\prime}(z) - g_{E^\prime}(\xi) ) \leq -\frac{1}{2}(1-\alpha) \gamma. 
\]
%
That is, can choose
%
\[
    \alpha \leq 
    \frac
        {\frac{1}{2}\gamma}
        {\frac{1}{2} \gamma + g_{E^\prime}(z_\mathrm{end})}
\]
where $z_\mathrm{end} \in \{\pm1\}$ maximises $g_{E^\prime}$ on $E$.

On the other hand, on $E^\prime$, we get asymptotic exponents of the form
\[
    -\frac
        {g_{E^\prime}(z_\mathrm{end})}
        {\frac{1}{2} \gamma + g_{E^\prime}(z_\mathrm{end})}
    \big[ 
        \gamma - \eta 
    \big]
        %
    - \frac
        {\frac{1}{2}\gamma}
        {\frac{1}{2} \gamma + g_{E^\prime}(z_\mathrm{end})}
    g_{E^\prime}(\xi) 
\]
But $g_{E^\prime}(\xi) \sim \mathsf{g}^\mathrm{def} + \beta^{-1}$ as $\mathsf{g} + \beta^{-1}\to0$ so this doesn't improve the asymptotic rates.

However, since $O(z) - I_N O(z)$ has $\alpha N$ zeros in $(\lambda-\ep,\lambda+\ep)$, for each $j \leq \alpha N$, we have
\[
    |O(z) - I_N O(z)| \leq C_j \bigg( \frac{\ep}{\alpha N} \bigg)^j |( O - I_NO)^{(j)}(\xi)| 
\]
for some $\xi \in (\lambda - \ep, \lambda + \ep)$.

\subsection{Instead: $E = [-1,a]\cup [\lambda-\ep,\lambda+\ep]\cup[b,1]$}
Here, we get 

\begin{figure}[htb]
    \centering
   
    \includegraphics[width=\textwidth]{diagrams/rates.png}
    \includegraphics[width=\textwidth]{diagrams/rates2.png}
        
    \caption{Left: Level sets $\{z\colon g_{E_j}(z) = g_{E_j}(\mu + i\pi\beta^{-1})\}$ for $E_1 = [-1,1]$ (red) $E_2 = [-1,a] \cup [b,1]$ (green) and $E_3 = [-1,a]\cup[\lambda-\ep,\lambda+\ep]\cup[b,1]$ (blue). The red dots are $\mu \pm i\pi\beta^{-1}$ Right: the corresponding asymptotic convergence rates $g_{E_j}(\mu + i\pi\beta^{-1})$. Dotted lines are $\sqrt{\mathsf{g}^2 + (\pi\beta^{-1})^2}$ and $\sqrt{(\mathsf{g}^{\mathrm{def}})^2 + (\pi\beta^{-1})^2}$}
\end{figure}
%

Seems to suggest that the asymptotic rate is somewhere between $\mathsf{g} + \beta^{-1}$ and $\mathsf{g}^\mathrm{def} + \beta^{-1}$. 

Actually, we have $\sqrt{\mathsf{g}^\mathrm{def}} + \beta^{-1}$ as $\mathsf{g} + \beta^{-1} \to 0$:
%
\begin{figure}[htb]
    \centering
   
    \includegraphics[width=\textwidth]{diagrams/sqrtEdge.png}
        
    \caption{Defect gap $\mathsf{g}^\mathrm{def}$ against the asymptotic convergence rate $g_E(\mu)$ (at zero temperature) on log-log plot. Dotted line is $\sqrt{\mathsf{g}^\mathrm{def}}$}
\end{figure}
%

\section{Pre-asymptotic Estimates}

If $f$ has zeros on $x_1,\dots,x_{n+1}$ then
\[
    f(x) = (x - x_1)(x_0^{(1)} - x_1^{(1)})(x_0^{(2)} - x_1^{(2)}) \dots (x^{(n-1)}_0 - x^{(n-1)}_1) f^{(n)}(x_0^{(n)})
\]
where
\begin{align}
    f(x) = f^\prime(x_0^{(1)}) (x - x_1) \quad \text{and} \\
    x_{k}^{(j)} \in (x_k^{(j-1)}, x_{k+1}^{(j-1)})
    \quad \text{with} \quad 
    f^{(j-1)}(x_k^{(j-1)}) - f^{(j-1)}(x_{k+1}^{(j-1)}) =  f^{(j)}( x_{k}^{(j)} ) (x_k^{(j-1)}) - x_{k+1}^{(j-1)})
\end{align}

If $x_j$ equally spaced then 
\[
    |f(x)| \leq n! h^n |f^{(n)}(\xi)|
\]
where $h$ is the spacing

\section{$L^2$ approximation error}

On Zulip: ``I've been trying various things but I think the most promising thing would be to instead consider the $L^2$ error. This gives at least as good error estimates from the potential theory + interpolation but the results may be better (this seems possible from numerical results). 

To do this, I used a weight function that is the characteristic function of the approximation domain $E$ and generated the orthonormal polynomials with respect to this weight. Then, we can take the best $L^2$ approximation $P_N$ on the space of polynomials of degree $N$. We have the estimate
\[
| [f(H) - P_N(H) ]_{\ell\ell} | 
%
\leq C \int_E | f(z) - P_N(z)| dz 
%
\leq C \| f - P_N \|_{L^2(E)} 
%
\leq C \inf_{Q_N} \| f - Q_N \|_{L^\infty(E)} 
\]
where the right hand side can be bounded using the potential theory estimates''

First inequality is wrong! 
\[
    [f(H) - P_N(H) ]_{\ell\ell} 
    %
    = \int \big( f(z) - P_N(z) \big) D_\ell(z)
    %
    = \int \big( f(z) - P_N(z) \big) \widetilde{D_\ell}(z) + \sum_s \big( f(\lambda_s) - P_N(\lambda_s) \big) [\psi_s]_\ell^2
\]

\section{Non-linearities}
Want
\[
    O(H)_{\ell\ell} \approx 
    %
    g\big( H_{\ell\ell}, [H^2]_{\ell\ell}, \dots, [H^N]_{\ell\ell} \big)
\]
($g$ linear $\to$ polynomial approximation $\to$ exponential rate but depends on defect)

%$g = \frac{g_1}{g_2}$ where $g_1,g_2$ are linear so that $RHS = \frac{P_N(H)_{\ell\ell}}{Q_N(H)_{\ell\ell}}$, then want to choose $P_N, Q_N$ such that
%\[
%   (f \cdot Q_N)(H)_{\ell\ell} - P_N(H)_{\ell\ell} %
%    \approx \sum_{k\not= \ell} f(H)_{\ell k} Q_N(H)_{k \ell}
%\]

Equivalent to: How well can we approximate $(z - H)^{-1}_{\ell\ell}$ with general functions of the variables
\[
    X_1 = H_{\ell\ell} 
    %
    \quad \text{and} \quad
    %
    X_n = \sum_{k_1,\dots,k_{n-1} \not= \ell} H_{\ell k_1}H_{k_1,k_2} \dots H_{k_{n-1}\ell}, \quad n \leq N
\]
?

For example: if $g$ is a power series 
\begin{align*}
    g(X_1,\dots,X_n) = \sum_{\bm{\alpha}} c_{\bm{\alpha}} X_{1}^{\alpha_1} \dots X_{N}^{\alpha_N}
\end{align*}
gives functions of the form
\begin{align*}
     g( H_{\ell\ell}, [H^2]_{\ell\ell}, \dots,  [H^N]_{\ell\ell} ) &= 
    %
    %\eqqcolon \sum_{n=0}^\infty a_n 
    %\sum_{
    %    \genfrac{}{}{0pt}{1}
    %        {t \text{ loop } \ell\to\ell}
    %        {\mathrm{len}(t) = n}
    %}
    %H_t \\
    %
    %&= \sum_{m = 0}^\infty 
    %\sum_{
    %    \bm{n} \in \mathbb N^m 
    %}
    %m! a_{|\bm{n}|_1} 
    %\sum_{
    %    \genfrac{}{}{0pt}{1}
    %        {t_j \text{ loop } \ell \to\ell \text{ only visiting $\ell$ at start and end}}
    %        {\mathrm{len}(t_j) = n_j}
    %}
    %H_{t_1} H_{t_2} \dots H_{t_m} \\
    %
     \sum_{n=0}^N a_n [H^{n}]_{\ell\ell} 
    %
    +\sum_{
        n_1 + n_2 \geq N+1
    } 
        a_{n_1, n_2}  
        [H^{n_1}]_{\ell\ell} [H^{n_2}]_{\ell\ell}
    %
    + \dots  \\
    %
    &\qquad\qquad \dots + \sum_{
        n_1 + \dots + n_m \geq (m-1)N + 1
    } 
    a_{n_1\dots n_m} [H^{n_1}]_{\ell\ell}
    [H^{n_2}]_{\ell\ell}\dots
    [H^{n_m}]_{\ell\ell} 
    %
    + \dots
\end{align*}
sum over loops $\ell\to\ell$ that can be written as a product of loops $\ell\to\ell$ each of length $\leq N$

(Not clear how to actually choose the parameters)

\iffalse
Bounds on the remainder: let $T$ be the set of all . Notation: if $t = (\ell\ell_1,\ell_1\ell_2, \dots, \ell_{n-1}\ell)$ is a loop $\ell \to \ell$ then write $H_t = H_{\ell \ell_1} \dots H_{\ell_{n-1}\ell}$. Therefore 
%
\begin{align}
    R_{N} &= 
    %
    \sum_{t \in T} a_{\mathrm{len}(t)} H_t 
    %
\end{align}
\fi


==> other/notes.tex <==
By the inclusion-exclusion principle, we have
    %
    \begin{align}
        (\Ham^n)_{\ell \ell} &= (\Ham_{\ell\ell})^n + \sum_{k \not=\ell } \Big( 
            \sum_{\ell_1, \dots, \ell_{n-1} \in \{\ell,k\}} \Ham_{\ell\ell_1} \Ham_{\ell_1\ell_2} \dots \Ham_{\ell_{n -1}\ell}
            %
            - (\Ham_{\ell\ell})^n
        \Big) \\
        %
        &\qquad+ 
        \sum_{k_1 < k_2 \colon k_1,k_2 \not=\ell } \Big( 
            \sum_{\ell_1, \dots, \ell_{n-1} \in \{\ell,k_1,k_2\}} 
            %
            - \sum_{\ell_1, \dots, \ell_{n-1} \in \{\ell,k_1\}} 
            %
            - \sum_{\ell_1, \dots, \ell_{n-1} \in \{\ell,k_2\}} 
            %
            + \sum_{\ell_1, \dots, \ell_{n-1} \in \{\ell\}} 
        \Big)
        + \dots
    \end{align}
    %
    Therefore, we have
    %
    \begin{align*}
        V_0^{(N)} &= I_N O( \Ham\big|_{\ell} )_{\ell \ell} 
        \\
        %
        V_1^{(N)}(\bm r_{\ell k}) &= \left[
            I_N O(\Ham\big|_{\ell;k}) - I_N O(\Ham\big|_{\ell})
        \right]_{\ell\ell} 
        %
        = I_N O(\Ham\big|_{\ell;k})_{\ell\ell} - V_0^{(N)} \\
        %
        V_2^{(N)}(\bm r_{\ell k_1}, \bm r_{\ell k_2}) &= \left[
            I_N O(\Ham\big|_{\ell;k_1k_2}) - I_N O(\Ham\big|_{\ell;k_1})- I_N O (\Ham\big|_{\ell;k_2})
            +I_N O(\Ham\big|_{\ell})
        \right]_{\ell\ell} \\
        %
        &= I_N O(\Ham\big|_{\ell;k_1k_2})_{\ell\ell} - V_1^{(N)}(\bm r_{\ell k_1}) - V_1^{(N)}(\bm r_{\ell k_2}) - V_0^{(N)}\\
        %
        \vdots\qquad\qquad &\qquad\qquad \vdots \\
        %
        V_n^{(N)}(\bm r_{\ell k_1}, \dots, \bm r_{\ell k_n}) 
        %
        &= I_N O( \Ham\big|_{\ell; k_1,\dots,k_n} )_{\ell \ell} 
        %
        - \sum_{K \subsetneqq \{k_1,\dots,k_n\}} V_{|K|}^{(n)}( \{ \bm r_{\ell k} \}_{k \in K} )
    \end{align*}



We have
    \begin{align*}
        V_1^{(N)}(\bm r_{\ell k}) &= \frac{1}{2\pi i} \oint_{\mathscr C} I_N O(z) 
        \Big[ 
            \big( \Ham\big|_{\ell;k} - z \big)^{-1} 
            \big( \Ham\big|_{\ell;k} - \Ham\big|_{\ell} \big) 
            \big( \Ham\big|_{\ell} - z \big)^{-1} 
        \Big]_{\ell\ell}\mathrm{d}z \\
        %
        V_2^{(N)}(\bm r_{\ell k_1},\bm r_{\ell k_2}) &= \frac{1}{2\pi i} \oint_{\mathscr C} I_N O(z) \Big[ 
            \big( \Ham\big|_{\ell;k_2} - z \big)^{-1} 
            \big( \Ham\big|_{\ell;k_1k_2} - \Ham\big|_{\ell;k_1} - \Ham\big|_{\ell;k_2} + \Ham\big|_{\ell}\big)
            \big( \Ham\big|_{\ell;k_1} - z \big)^{-1} \\
            %
            &\qquad\qquad 
            %
            - \big( \Ham\big|_{\ell;k_1k_2} - z \big)^{-1}
            \big( \Ham\big|_{\ell;k_1k_2} - \Ham\big|_{\ell;k_2}\big)
            \big( \Ham\big|_{\ell;k_2} - z \big)^{-1}
            \big( \Ham\big|_{\ell;k_1k_2} - \Ham\big|_{\ell;k_1}\big)
            \big( \Ham\big|_{\ell;k_1} - z \big)^{-1}\\
            %
            &\qquad\qquad 
            %
            - \big( \Ham\big|_{\ell;k_2} - z \big)^{-1}
            \big( \Ham\big|_{\ell;k_2} - \Ham\big|_{\ell}\big)
            \big( \Ham\big|_{\ell;k_1} - z \big)^{-1}
            \big( \Ham\big|_{\ell;k_1} - \Ham\big|_{\ell}\big)
            \big( \Ham\big|_{\ell} - z \big)^{-1}
        \Big]_{\ell \ell} \mathrm{d}z
    \end{align*}
    where $\mathscr C$ is a simple closed contour encircling the spectrum (e.g.~choosing an equi-potential contour as in Fig~1 gives the boundedness of the integrand).
    
    
    
\subsection{Eigenvalues in the gap}

Suppose we have a point defect and consider defect Hamiltonian $\Ham^\mathrm{def}$ and defect-free Hamiltonian $\Ham$. Then, suppose $\lambda$ is an eigenvalue in the gap. 

What properties does $\lambda$ satisfy? body-order, truncate environment? ...

For a simple closed positively oriented contour $\mathscr C_\lambda$ encircling $\lambda$ and avoiding the rest of the spectrum, we have

\begin{align}
    \lambda &= \sum_\ell \lambda |\psi_\ell|^2 = - \mathrm{Tr}\, \frac{1}{2\pi i} \oint_{\mathscr C_\lambda} (\Ham^\mathrm{def} - z)^{-1}\\
    %
    &= - \mathrm{Tr}\, \frac{1}{2\pi i} \oint_{\mathscr C_\lambda} 
    \big[ 
        (\Ham^\mathrm{def} - z)^{-1} - (\Ham - z)^{-1} 
    \big]\mathrm{d}z \\
    %
    &= - \sum_{\ell \in \mathrm{DEF}} \frac{1}{2\pi i} \oint_{\mathscr C_\lambda} 
    \big[ 
        (\Ham^\mathrm{def} - z)^{-1} - (\Ham - z)^{-1} 
    \big]_{\ell\ell} \mathrm{d}z + O(e^{-\gamma r_\mathrm{cut}})
\end{align}
%
Suffices to show that we can write the resolvents themselves as body-order expansions. To do this, we let $\mathscr C$ be a system of simple closed contours encircling $\sigma(\Ham)$ and avoiding $\{z\}$ (picture below) and write
%
\begin{align}
    (\Ham - z)^{-1} &= -\frac{1}{2\pi i} \oint_{\mathscr C} \frac{1}{\xi - z} (\Ham - \xi)^{-1} \mathrm{d}\xi \\
    %
    &\approx -\frac{1}{2\pi i} \oint_{\mathscr C} P_N(\xi; z) (\Ham - \xi)^{-1} \mathrm{d}\xi
    %
    = P_N(\Ham; z)
\end{align}
Here, it is possible to approximate $\xi \mapsto \frac{1}{\xi - z}$ by polynomials uniformly on compact neighbourhoods of $\sigma(\Ham))$. (This is exactly what we are doing when we approximate $F_\beta$ along contours that encircle the spectrum and avoid the poles at $\mu \pm i\pi\beta^{-1}$)


\begin{figure}[htb]
      \centering
      \includegraphics[width=.9\textwidth]{diagrams/resolvent expansion.jpg}
\end{figure}


We therefore obtain 
\begin{align}
    \lambda &= \sum_{\ell \in \mathrm{DEF}} \frac{1}{2\pi i} \oint_{\mathscr C_\lambda} 
    \big[ 
        P_N(\Ham;z) - P_N(\Ham^\mathrm{def};z)  
    \big]_{\ell\ell} \mathrm{d}z 
    %
    + O(e^{-\gamma r_\mathrm{cut}}) 
    %
    + O(e^{-\eta N}) \\
    %
    &= \sum_{\ell \in \mathrm{DEF}} [Q_N(\Ham) - Q_N(\Ham^\mathrm{def})]_{\ell\ell} + O(e^{-\gamma r_\mathrm{cut}}) 
    %
    + O(e^{-\eta N}) 
\end{align}
Again, we can truncate the atomic environment around $\ell$ and get another exponentially small error

Questions
\begin{itemize}
    \item How does the error in the interpolation nodes carry over to the interpolations: for small $\ep > 0$, can we write
    \[
        | I_{X \cup \{x\} }O_\ell(\bm r) - I_{X \cup \{x + \ep\} }O_\ell(\bm r) | \leq C \ep ?
    \]
    
    \item Are methods (iii) and (iv) essentially equivalent? Do we get the same error bounds if we instead define
    \[
        O_\ell^N(\bm r) \coloneqq \frac{1}{2\pi i} \oint O(z) P_N(\Ham;z)_{\ell\ell} \mathrm{d}z?
    \]
    Or does the fact that we need a polynomial for each point along the contour improve the estimate at all?
    
    \item Can we rigorously prove that classical body-order expansion is bad? Why is it so bad if it is more complicated than a simple polynomial? What ``type'' of function is it in terms of the powers $\Ham_{\ell\ell}, [\Ham^2]_{\ell\ell},\dots,[\Ham^N]_{\ell\ell}$?
    
    \item Does allowing approximations of the form $\frac{P_N(\Ham)_{\ell\ell}}{Q_N(\Ham)_{\ell\ell}}$ improve the estimates?
    
    \item What happens if we did a combination of approximating $z \mapsto O(z)$ and the resolvent?
\end{itemize}

%%%%%%%%%%% POINT DEFECTS REMARK %%%%%%%%%%%%%
\begin{remark}[Point defects]\label{rem:point-defs-1}
We now briefly describe the particular case of point defects embedded in a perfect crystal. If 
%
$\bm{r}^\# = \{\bm{r}^{\#}_\ell\}_{\ell \in \Lambda^\#}$ 
%
represents multi-lattice and the potential 
%
$v^{\#}= \{v^{\#}_\ell\}_{\ell \in \Lambda^\#}$ 
%
has the same periodicity, then a simple application of Bloch's theorem \cite{bk:kittel} reveals that the spectrum 
%
$\sigma\big( \Ham(\bm{r}^{\#}, v^{\#}) \big)$ 
%
is the union of finitely many continuous energy bands. A point defect can be described by an index set 
%
$\Lambda \coloneqq \Lambda_{\mathrm{def}} \cup \Lambda_{\mathrm{ff}}$, 
%
atomic positions 
%
$\bm{r} = \{\bm{r}_\ell\}_{\ell\in \Lambda}$
%
and the potential
%
$v = \{v_\ell\}_{\ell\in \Lambda}$ 
%
such that $\Lambda_{\mathrm{def}}$ is finite, 
%
$\Lambda_{\mathrm{ff}} = \Lambda \setminus \Lambda_0$
%
for some finite set $\Lambda_0$ and 
%
\[
    \bm{r}_\ell = \bm{r}^\#_\ell 
    %
    \quad \text{and} \quad 
    %
    v_\ell = v_\ell^\# \quad \text{for all } \ell \in \Lambda_{\mathrm{ff}}.
\]
%

In this setting, we apply the Weyl perturbation theorem \cite{bk:Kato1995} to conclude that the essential spectrum of $\Ham( \bm{r} , v )$ is equal to
%
$\sigma\big( \Ham( \bm{r}^\# , v^\# ) \big)$.
%
Moreover, there are at most finitely many additional eigenvalues bounded away from the spectrum \cite{OrtnerThomas2020:pointdefs}: for all $\delta > 0$, 
%
\[
    \left|\sigma\big( \Ham( \bm{r} , v ) \big) \setminus 
        B_\delta\big( \sigma\big( \Ham( \bm{r}^\# , v^\# ) \big) \big)\right|
    < \infty.
\]
%

\jt{Actually, as it stands, $\Ham(\bm r, v)$ is a finite rank update of $\Ham(\bm r^\#, v^\#)$. This result is true for finite energy displacements of the point defect reference and more general effect potentials (only need $|v_\ell - v_\ell^\#| \to 0$ as $|\ell|\to\infty$)}

\jt{need to check this is true for 3C case - this seems obvious - maybe we can say so and cite the 2C case}

Therefore, if $\bm{r}^\#$ represents an insulator, then the results of Theorem~\ref{thm:bodyOrder_interpolation_discrete} hold for $\bm{r}$. In addition, we may apply the low-rank perturbation results of \cite{ChenOrtnerThomas2019:locality} to conclude that the exponent $\widetilde{\gamma}_N$ can be chosen to be equal the corresponding exponent $\gamma_N$ from Theorem~\ref{thm:bodyOrder_interpolation}. In doing this, the pre-factor $\widetilde{C}$ increases and depends on the atomic site $\ell$. Moreover, this pre-factor converges to the corresponding defect-free pre-factor from Theorem~\ref{thm:bodyOrder_interpolation} as $|\bm{r}_\ell|\to\infty$, with an exponential rate.
\end{remark}

==> other/oldProof25.tex <==



\begin{proof}[Proof of Theorem~\ref{thm:trun-nbh_int}]

     We define 
     %
     $P \coloneqq \Ham(\bm{r},v) - \widetilde{\Ham}^{r_\mathrm{c}}(\bm{r},v)$
     %
     to be the ``far-field'' perturbation, simplify notation by writing 
    %
    $\mathscr R_z \coloneqq 
    \big( 
        \Ham(\bm{r},v) - z
    \big)^{-1} 
    %
    = \big( 
        \widetilde{\Ham}^{r_\mathrm{c}}(\bm{r},v) + P - z
    \big)^{-1}$
    and 
    %
    $\widetilde{\mathscr R}_z \coloneqq \big(         
        \widetilde{\Ham}^{r_\mathrm{c}}(\bm{r},v) - z
    \big)^{-1}$.
    %
    In order to estimate the difference between the local quantity of interest and the corresponding sparse approximation, we consider the difference between the two resolvent operators:
    %
    \begin{align}\label{eq:woodbury}
       \mathscr R_z - \widetilde{\mathscr R}_z 
       %
       &= - \widetilde{\mathscr R}_z
       \big(
            I + P \widetilde{\mathscr R}_z
       \big)^{-1}
       P \widetilde{\mathscr R}_z 
       %
     % = \widetilde{\mathscr R}_z - \widetilde{\mathscr R}_z P
     %  \big(
     %       I + \widetilde{\mathscr R}_z P
     %  \big)^{-1}
     %  \widetilde{\mathscr R}_z
    \end{align}
    %
    where the matrix entries of 
    %
    $\big(
            I + P\widetilde{\mathscr R}_z
    \big)^{-1} 
    %
    = (\widetilde{\Ham} - z) \mathscr R_z$ 
    %
    are uniformly bounded for $z$ in a bounded set. The update formula \cref{eq:woodbury} (but for low rank perturbations) is the key ingredient for the improved locality estimates in the case of point defects
    %
    \cite{
        ChenOrtnerThomas2019:locality,
        Thomas2020:scTB
    }.
    %
    
    Applying the Hermite integral formula \cref{eq:Hermite:prelim} directly, we conclude that $I_NO^\beta(z)$ is bounded uniformly in $N$ along a suitably chosen contour $\mathscr C \coloneqq \{ g_E = \gamma \}$ (examples of such contours are given in Figure~\ref{fig:equipot}). 
    %
    It is important to note that the contour $\mathscr C$ must be chosen to encircle both $\sigma(\Ham)$ and $\sigma( \widetilde{\Ham} )$. 
    %
    In the following, we let $\gamma_\mathrm{CT}$ be the Combes-Thomas exponent from Lemma~\ref{lem:CT}. 
    %

    Therefore, using \cref{eq:woodbury} together with \textit{(T3)}, we conclude
    %
    \begin{align}
        \left|
            I_N O^\beta_\ell(\bm{r},v) - I_N \widetilde{O}^\beta_\ell(\bm{r},v)      
        \right| 
        %
        &= \frac{1}{2\pi} \left| \oint_{\mathscr C} I_N O^\beta(z) \sum_a
        \big[
            \mathscr R_z - \widetilde{\mathscr R}_z 
        \big]_{\ell\ell}^{aa} \mathrm{d}z \right| 
            \nonumber\\
        %
        &\leq C \max_{z\in\mathscr C} \|\big(
            I + \widetilde{\mathscr R}_z P
       \big)^{-1}\|_{\mathrm{max}} 
       %
       \sum_{k_1,k_2,k_3}
        e^{-\gamma_\mathrm{CT} r_{\ell k_1}} |P_{k_2 k_3}| e^{- \gamma_\mathrm{CT} r_{k_3 \ell}} 
            \nonumber \\ 
        %
        &\leq C e^{- c_0 \min\{\gamma_0, \gamma_\mathrm{CT}\} \, r_\mathrm{c}}. \label{eq:truncation-pf}
    \end{align}
    This concludes the proof.
\end{proof}
%    

==> other/questions.tex <==
\section{Questions}
\begin{itemize} 

    \item Throughout, we have assumed a fixed chemical potential \cite{ChenLuOrtner18}. But for the convergence of the approximation scheme, the fixed chemical potential given by the self-consistent density is unknown. Is it worth proving that the chemical potential $\mu^n$ corresponding to $\rho^n$ converges as $n\to\infty$ to the chemical potential corresponding to $\rho^\star$... 

    \item \textcolor{red}{The equation $\rho = F(u,v)$ only makes sense for a very limited number of infinite systems. i.e.~for Yukawa, or Coulomb where $\rho_\ell = Z_\ell$ for all $\ell$}
    
    \item Derive minimisation problem for finite systems and for Yukawa
    
     \begin{align}
        \rho^R &\in \argmin  E[\rho]  \\
        %
        E[\rho] &\coloneqq 2\mathrm{Tr} \rho H_0
        - \sum_{\ell \not= k} \frac{\rho_\ell Z_{k}}{r_{\ell k}}
        + \frac{1}{2} \sum_{\ell \not= k} \frac{\rho_{\ell} \rho_{k}}{r_{\ell k}} + \frac{2}{\beta}\sum_s S(f_s) + E_{ZZ} \\
        %
        \rho_{\ell k} &= \sum_s f_s [\psi_s]_\ell[\psi_s]_k, \qquad \rho_\ell \coloneqq \rho_{\ell\ell},
        %
        \qquad \mathrm{Tr} \rho = |\Lambda|
    \end{align}
    
    where $H_0$ is only the linear part of the Hamiltonian and $S(f) = f \log f + (1 - f) \log (1-f)$ is the entropy.
    
    \begin{itemize}
        \item Is this the ``right'' energy? Extra bit should resemble $- \int \rho V_\mathrm{ext} + \frac{1}{2}\int \rho V_\mathrm{H}$ from DFT since we are neglecting the exchange correlation energy. Then, at finite temperature so need the entropy contribution.
        
        \item Existence and Uniqueness? Proved for restricted Hartree-Fock and this is just a discretised version
        
        \item Do minimisers satisfy $\rho_\ell = f_\beta( H[\rho] - \mu )_{\ell\ell}$? i.e. do we have $f_s = f_\beta(\lambda_s - \mu)$ where $\lambda_s$ is an eigenvalue of the non-linear Hamiltonian?
        
        \item Renormalise and take thermodynamic limit. Derive a periodic problem with renormalised Coulomb potential? 
        \item Hope that minimum energy and minimising densities converge to a corresponding periodic problem with $\frac{1}{r_{\ell k}}$ replaced with some $G_{\ell k}$
        
        \item These questions have been solved for TF, TFvW and rHF [Catto, Le Bris, Lions, '98, '00, etc]. E.g.~in HF, the electrostatic potential created by the nuclei is replaced with $G$ periodic and solving 
        \[
            - \Delta G = 4\pi \bigg( 
                \sum_{y \in \Lambda} \delta( \,\cdot - y) - 1
            \bigg)
        \]  
        with mean zero $\int_Q G = 0$. We have, 
        \[
            G(x) = \sum_{k} \left( 
                \frac{1}{| x - k|} - \int_\Gamma \frac{1}{|x - (k + y)|}\mathrm{d}y
            \right) - d
        \]
        for some constant $d$ independent of the sequence of domains $\Lambda \to \infty$. They then prove that thermodynamic limit of the finite problem converges to same model but with Coulomb replaced with $G$
        
        \item Then consider defects
        
        \item Combine with geometry optimisation: For a sequence of domains $\Lambda \to \infty$, do limits of ground state electron densities for the optimised geometries converge? 
    \end{itemize}
    
    \item does this also agree with Yukawa exponent $\to 0$?
    
    \item Under what circumstances can we iteratively solve $\rho = I_N \widetilde{F}(\bm{r};\rho)$? If there exists stable solution, then Newton iteration works. Can we strengthen this result by using simpler mixing strategies.
    
    \item COnvergence result $\rho^n \to \rho^\star$ for $\rho^n = \rho^n(N(n), r_\mathrm{cut}(n))$ with $N(n), r_\mathrm{cut}(n) \to \infty$ in for Coloumb.
    
    \item Zero temperature limit?
\end{itemize}
